The Heat is On: Thermal Facial Landmark Tracking

Facial landmark tracking for thermal images requires tracking certain important regions of subjects' faces, using images from thermal images, which omit lighting and shading, but show the temperatures of their subjects. The fluctuations of heat in particular places reflect physiological changes like bloodflow and perspiration, which can be used to remotely gauge things like anxiety and excitement. Past work in this domain has been limited to only a very limited set of architectures and techniques. This work goes further by trying a comprehensive suit of various models with different components, such as residual connections, channel and feature-wise attention, as well as the practice of ensembling components of the network to work in parallel. The best model integrated convolutional and residual layers followed by a channel-wise self-attention layer, requiring less than 100K parameters.

==> vqgan.tex <==
\subsubsection{VQGAN}
Inspired by architecture from \cite{ho2020denoising}, who described their method as a ''U-Net with self attention'', \cite{esser2020taming} used a VQGAN for developing crisp, realistic images for maximum activation of nodes that corresponded to various classes (cats, dogs, etc). The novelty of their generation pipeline was an Encoder \(E\) that mapped input images to latent space representations, so that
\begin{equation}
E(x):\mathbb{R}^{H \times W \times C} \rightarrow \mathbb{R}^{h \times w \times z}
  \label{eq:encoder}
\end{equation}
followed by a Decoder \(D\) that mapped latent space image representations so that
\begin{equation}
D(x): \mathbb{R}^{h \times w \times z} \rightarrow \mathbb{R}^{H \times W \times C}
  \label{eq:decoder}
\end{equation}
At a high level, the Encoder would downsample the input images and then apply attention, while the Decoder would apply attention and then upsample. Given that \(h <<< H, w <<< W, C <<< z\), this was a less computationally expensive, but more feature-sensitive way to do attention than performing attention on an entire image, and is similar to the approach in this paper and others \cite{xu2016show}.
